Small random initialization is akin to spectral learning: Optimization and generalization guarantees for overparameterized low-rank matrix reconstruction

Recently there has been significant theoretical progress on understanding the convergence and generalization of gradient-based methods on nonconvex losses with overparameterized models. Nevertheless, many aspects of optimization and generalization and in particular the critical role of small random initialization are not fully understood. In this paper, we take a step towards demystifying this role by proving that small random initialization followed by a few iterations of gradient descent behaves akin to popular spectral methods. We also show that this implicit spectral bias from small random initialization, which is provably more prominent for overparameterized models, also puts the gradient descent iterations on a particular trajectory towards solutions that are not only globally optimal but also generalize well. Concretely, we focus on the problem of reconstructing a low-rank matrix from a few measurements via a natural nonconvex formulation. In this setting, we show that the trajectory of the gradient descent iterations from small random initialization can be approximately decomposed into three phases: (I) a spectral or alignment phase where we show that that the iterates have an implicit spectral bias akin to spectral initialization allowing us to show that at the end of this phase the column space of the iterates and the underlying low-rank matrix are sufficiently aligned, (II) a saddle avoidance/refinement phase where we show that the trajectory of the gradient iterates moves away from certain degenerate saddle points, and (III) a local refinement phase where we show that after avoiding the saddles the iterates converge quickly to the underlying low-rank matrix. Underlying our analysis are insights for the analysis of overparameterized nonconvex optimization schemes that may have implications for computational problems beyond low-rank reconstruction.

==> notation.tex <==
\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline}
%\usepackage[]{algorithm2e}
\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{4}

\titleformat{\paragraph}
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing*{\paragraph}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\usepackage{movie15}

\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bt}{\bigotimes}
%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{I}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
\newcommand{\E}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}


==> outlook.tex <==
\section{Outlook}\label{section:outlook}

\textcolor{red}{Dominik: Should we write something there?}


\section*{Acknowledgements}
D. St\"oger is supported by the Air Force Office of Scientific Research under award \#FA9550-18-1-00788. M. Soltanolkotabi is supported by the Packard Fellowship in Science and Engineering, a Sloan Research Fellowship in Mathematics, an NSF-CAREER under award \#1846369, the Air Force Office of Scientific Research Young Investigator Program (AFOSR-YIP) under award \#FA9550-18-1-0078, DARPA Learning with Less Labels (LwLL) and FastNICS programs, and NSF-CIF awards \#1813877 and \#2008443.\textcolor{red}{DS: @Mahdi: Please check whether this is correct}.

==> rest.tex <==



\section{Main results}\label{sec:mainresults}

In this section, we present our main results. Stating these results requires a couple of simple definitions. The first definition concerns the measurement operator $\mathcal{ A}$. %Specifically, we assume that it satisfies the restricted isometry property, which is defined as follows.
\begin{definition}[Restricted Isometry Property (RIP)]\label{def:restrictedisometry}
The measurement operator $\mathcal{ A}: \R^{n\times n} \longrightarrow \mathbb{R}^m$ satisfies RIP of rank $r$ with constant $\delta>0$, if it holds for all matrices $Z$ of rank at most $r$
\begin{equation}\label{equation:RIP}
\left(1-\delta \right) \fronorm{Z}^2 \le  \twonorm{ \mathcal{ A} \left(Z\right)  }^2  \le \left(1+\delta \right) \fronorm{Z}^2.
\end{equation}
\end{definition}
We note that for a Gaussian measurement operator $\mathcal{ A}$ 
\footnote{By that, we mean that all the entries of the (symmetric) measurement matrices $\left\{ A_i \right\}_{i=1}^m$ are drawn i.i.d. with distribution $\mathcal{ N} \left(0,1\right) $ on the off-diagonal and distribution $ \mathcal{ N} \left(0,1/\sqrt{2}\right)  $ on the diagonal.},
RIP of rank $r$ and constant $\delta >0$ holds with high probability, if the number of observations satisfies $ m \gtrsim  nr/\delta^{2} $ \cite{candesplan, vershynin2018high}.

The second definition concerns the condition number of the factor $X$.
\begin{definition}[condition number] We denote the condition number of $X \in \mathbb{R}^{n \times r_{\star}}$ by  $
\kappa:= \frac{\specnorm{X}}{\sigma_{r_{\star} } \left(X\right)}
$,
where $\sigma_{r_{\star} } \left(X\right)$ denotes $r_{\star}$-th largest singular value of $X$.
\end{definition}
With these definitions in place we are now ready to state our main results. Due to space limitations in the main paper we focus on the case of $ r\ge 2r_{\star} $. With refer the reader to the supplementary for results covering all $r\ge r_{\star}$ including two special cases: (1) the fully overparameterized case, i.e., $r= n$ along with comparisons with existing work, in this case \cite{LiMaCOLT18}, and (2) the scenario that $U$ has the same number of parameters as $X$, i.e., $r=r_{\star}$.
\begin{theorem}\label{mainresult:runequaln} 
	Let $X\in\R^{n\times r_*}$ and assume we have $m$ measurements of the low rank matrix $XX^T$ of the form $y = \mathcal{ A}\left(XX^T\right)$ with $\mathcal{ A}$ the measurement operator. We assume $\mathcal{ A}$ satisfies the restricted isometry property for all matrices of rank at most $2r_{\star}+1$ with constant $\delta \le  c \kappa^{-4} {r_{\star}}^{-1/2}    $. To reconstruct $XX^T$ from the measurements we fit a model of the form $\bar{U}\mapsto\mathcal{ A}\left(\bar{U}\bar{U}^T\right)$ with $\bar{U}\in\R^{n\times r}$ and $r>r_*$ via running gradient descent iterations of the form $U_{t+1} = U_t - \mu \nabla f \left(U_t\right)$ on the objective \eqref{mainopt} with a step size obeying $ \mu \le c \kappa^{-4} \specnorm{X}^{-2}  $. Here, the initialization is given by $U_0 =  \alpha U$, where $U \in \mathbb{R}^{n \times r}$ has  i.i.d. entries distributed as $ \mathcal{ N} \left(0, 1/\sqrt{r} \right) $.  Furthermore, we assume $r \ge 2 r_{\star} $ and that  the scale of initialization fulfills 
		\begin{equation}\label{ineq:alphabound}
		%\alpha \le  \min \left\{ \frac{  \left( \min \left\{ r;n  \right\} \right)^{1/2}     }{      \kappa^{1/2} n^{3/4}}; \frac{1}{\min \left\{ r;n  \right\}}  \right\}   \left(     2 \kappa^2  \sqrt{\frac{n}{\min \left\{ r;n  \right\}}}   \right)^{-6\kappa^2}  \specnorm{X} .
			\alpha \lesssim  \min \left\{ \frac{  \left( \min \left\{ r;n  \right\} \right)^{1/2}     }{      \kappa^{1/2} n^{3/4}}  \left(     2 \kappa^2  \sqrt{\frac{n}{\min \left\{ r;n  \right\}}}   \right)^{-6\kappa^2} ; 		  \frac{  \min \left\{ r;n \right\} }{\kappa^7 n^2 }\right\}   \specnorm{X} .
		\end{equation}
		Then,  after 
		\begin{align*}
		\hat{t} \lesssim \frac{1}{\mu \sigma_{ \min }  \left(X\right)^2}  \ln \left(  \frac{ C_1 n\kappa }{\min \left\{ r;n  \right\}}  \cdot  \max \left\{   1; \frac{\kappa r_{\star}}{\min \left\{ r;n  \right\}-r_{\star}} \right\}   \cdot   \frac{ \Vert X \Vert}{\alpha} \right)
		\end{align*}
		iterations we have that
		\begin{equation}\label{ineq:generalizationerror1}
		\frac{\fronorm{ U_{\hat{t}} U_{\hat{t}}^{T} - XX^T  }   }{\specnorm{X}^2} \lesssim    \frac{  n^2  \kappa^{81/16}    r_{\star}^{1/8}  }{   \left( \min \left\{ r;n \right\} \right)^{5/8}  }   \cdot  \frac{   \alpha^{21/16}  }{  \specnorm{X}^{21/16}},
		\end{equation}
		holds with probability at least $ 1 - C e^{-\tilde{c} r  }$. % with $\tilde{c} $ and $C$ fixed numerical constants.
 Here, $C_1, C_2, \tilde{C}, \tilde{c}>0$ are fixed numerical constants.%absolute constants chosen large enough.
\end{theorem}
Note that the test error $ \fronorm{U_{\hat{t}} U_{\hat{t}}^{T}  -XX^T  }^2 $ can be made arbitrarily small by choosing the scale of initialization $\alpha$ small enough. In particular, the dependence of the test error on $\alpha$ is polynomial and the dependence of the  number of iterations on $\alpha$ is logarithmic, which means  that reducing the test error by scaling down $\alpha$  introduces only modest additional computational cost. Hence, as long as the rank at most $2r_{\star}+1$ RIP with constant $\delta \le  c \kappa^{-4} {r_{\star}}^{-1/2} $ holds, gradient descent converges to a point in the proximity of the low-rank solution, whenever the initialization is chosen small enough regardless of the choice of $r$. This holds even when the model is overparameterized i.e.~$ rn \gg m  $ and the optimization problem has many global optima many of which do not obey $UU^T\approx XX^T$. This result thus further demonstrates that when initialized with a small random initialization gradient descent has an implicit bias towards solutions of low-rank or small nuclear norm. This is in sharp contrast to Neural Tangent Kernel (NTK)-based theory for  low-rank matrix recovery (see \cite[Section 4.2]{oymak2019overparameterized}) which will not approximately recover the ground truth matrix $XX^T$ due to the larger scale of initialization required when using that technique.

As discussed in Section \ref{section:lowrankmatrixrecovery}, the restricted isometry property holds with high probability for a sample complexity $ m \gtrsim nr_{\star}^2 \kappa^{8}$ for Gaussian measurement matrices. Up to constants, this sample complexity %$nr_{\star}^2 \kappa^{8}$ %n Theorem \ref{mainresult:runequaln}
 is optimal in $n$, while it is sub-optimal in $r_{\star}$ and $\kappa$ compared to approaches based on nuclear-norm minimization (see, e.g., \cite{candesplan}). While there is numerical evidence that the true scaling of $m$ in $r_{\star}$ should also be linear in the non-convex case \cite{bhojanapalli2016global}, we note that the optimal dependence of the sample complexity on $r_{\star}$ is a major open problem in the field, as the sample complexities in all theoretical results for non-convex approaches in the literature scale at least quadratically in $r_{\star}$. 

%Moreover, note that while in the theorem above we have assumed that $\mathcal{ A}$ is a Gaussian measurement operator, it will become clear from our proofs that this assumption can be significantly weakened -- the only assumption on the measurement operator $\mathcal{ A}$, which we are going to use in our proofs is that the measurement operator $\mathcal{A}$ fulfills the restricted isometry property of order $2r_{\star}$ with a constant $ \delta \lesssim nr^{-1/2} \kappa^{-4}  $.\\
% 

\textbf{Interpretation: } %It is interesting to see how the result changes, when the parameter $r$ is varied, i.e., the number of parameters changes. 
Recall from Section \ref{section:introduction} that our convergence analysis can be divided into three phases: the spectral phase, the saddle avoidance phase, and the local refinement phase. As it will become clear from the proofs in the supplementary when $r \ge 2r_{\star} $ the bound on the number of iterations can be decomposed as follows 
{\small
 \begin{equation}\label{ineq:iterationsdecomposition}
 \begin{split}
%\hat{t} \lesssim & \bracing{\text{Phase I: spectral/alignment phase}}{\frac{1}{\mu \sigma_{ \min }  \left(X\right)^2}  \ln \left(     2 \kappa^2  \sqrt{\frac{n}{\min \left\{ r;n \right\}}}    \right)} + \bracing{\text{Phase II: saddle avoidance phase}}{\frac{1}{\mu \sigma_{ \min }  \left(X\right)^2}    \ln \left(\frac{ \sigma_{ \min } \left(X\right) }{\alpha} \right)} \\
% &+ \bracing{\text{Phase III:  local refinement phase}}{ \frac{1}{\mu \sigma_{ \min }  \left(X\right)^2}    \ln \left( \max \left\{   1; \frac{\kappa r_{\star}}{r-r_{\star}} \right\}   \frac{ \Vert X \Vert}{\alpha} \right) }.
\hat{t} \lesssim & \frac{1}{\mu \sigma_{ \min }  \left(X\right)^2}  \Bigg\lbrack   \bracing{\text{Phase I: spectral/alignment phase}}{ \ln \left(     2 \kappa^2  \sqrt{\frac{n}{\min \left\{ r;n \right\}}}    \right)} + \bracing{\text{Phase II: saddle avoidance phase}}{  \ln \left(\frac{ \sigma_{ \min } \left(X\right) }{\alpha} \right)} + \bracing{\text{Phase III:  local refinement phase}}{    \ln \left( \max \left\{   1; \frac{\kappa r_{\star}}{\min \left\{ r;n \right\} -r_{\star}} \right\}   \frac{ \Vert X \Vert}{\alpha} \right)   } \Bigg\rbrack  .
\end{split}
 \end{equation}
 }
 First, we note that the duration of all three phases scales inversely with $ \sigma_{ \min  } \left(X\right)^2 $. This is due to the fact that in all three phases the dynamics associated the smallest singular value of $X$ is the slowest one and hence needs the most time to complete.
 
 In the spectral phase,  the eigenvectors corresponding  to the  leading $r_{\star}$ eigenvalues of $\UUt \UUt^T$ become aligned with the eigenvectors corresponding  to the  leading $r_{\star}$ eigenvalues of $\mathcal{ A}^* \mathcal{ A} \left(XX^T\right)$. We observe in \eqref{ineq:iterationsdecomposition}  that in the spectral phase increasing $r$, i.e. the amount of parameters, decreases the number of iterations in this phase. As we will explain in the supplementary, the reason is that increasing $r$ decreases the angle between the column space of the initialization $U_0$ and the span of the eigenvectors corresponding to the leading $r_{\star}$ eigenvalues of $\mathcal{ A}^* \mathcal{ A} \left(XX^T\right)$ used in spectral initialization. As a consequence, gradient descent needs fewer iterations to align these two subspaces. %Note that for this reason, in the case of smaller $r$,  also a smaller scale of initialization $\alpha$ is required, see assumption \eqref{ineq:alphabound}.
 
In the saddle avoidance phase (Phase II), $\sigma_{r_{\star} }\left( \UUt \right) $ , the $r_{\star}$th largest singular value of $\UUt$, grows geometrically until it is on the order of $ \sigma_{ \min  } \left(X\right) $. Hence, this duration depends on the ratio between the $\sigma_{ \min  } \left(X\right) $ and the the scale of initialization $\alpha$. This is clearly reflected in the upper bound on the number of needed iterations in equation \eqref{ineq:iterationsdecomposition}.

 In Phase III, the local refinement phase, the matrix $ \UUt \UUt^T $ converges towards $ XX^T $. In particular, at iteration $\hat{t}$ the test error obeys \eqref{ineq:generalizationerror1}. We observe that a smaller $\alpha$ allows for a smaller test error in \eqref{ineq:generalizationerror1} but per \eqref{ineq:iterationsdecomposition} this higher accuracy is achieved with a modest increase in the required iterations.
 
 %Furthermore, we also see that increasing $r$ results in fewer iterations in Phase III and, hence, if one increases $r$ the total number of iterations $\hat{t}$ is decreasing. Note that also the generalization error \eqref{ineq:generalizationerror1} is decreasing in $r$. Hence, when one increases the number of columns $r$ of $\UUt$, Theorem \ref{mainresult:runequaln} guarantees a smaller generalization error with fewer iterations.
 
 %This decomposition also shows in the refinement phase decreasing the initialization scale $\alpha$ increases the number of gradient descent iterations but leads to a smaller generalization error $ \fronorm{ U_{\hat{t}} U_{\hat{t}}^{T} -XX^T }  $.  %However, let us stress that numerical simulations \cite{LiMaCOLT18} indicate that early stopping at iteration $\hat{t}$  is not required. Indeed, the gradient descent algorithm reaches a small error floor and the error will not go up, even after a large number of iterations.

